Application-level Studies of Cellular Neural Network-based Hardware Accelerators

As cost and performance benefits associated with Moore's Law scaling slow, researchers are studying alternative architectures (e.g., based on analog and/or spiking circuits) and/or computational models (e.g., convolutional and recurrent neural networks) to perform application-level tasks faster, more energy efficiently, and/or more accurately. We investigate cellular neural network (CeNN)-based co-processors at the application-level for these metrics. While it is well-known that CeNNs can be well-suited for spatio-temporal information processing, few (if any) studies have quantified the energy/delay/accuracy of a CeNN-friendly algorithm and compared the CeNN-based approach to the best von Neumann algorithm at the application level. We present an evaluation framework for such studies. As a case study, a CeNN-friendly target-tracking algorithm was developed and mapped to an array architecture developed in conjunction with the algorithm. We compare the energy, delay, and accuracy of our architecture/algorithm (assuming all overheads) to the most accurate von Neumann algorithm (Struck). Von Neumann CPU data is measured on an Intel i5 chip. The CeNN approach is capable of matching the accuracy of Struck, and can offer approximately 1000x improvements in energy-delay product.

==> temp.tex <==
This implementation uses a predefined sequence of the kernels and the object tracking is based mostly on motion and change detection. 
Tracking based on motion detection can perform well on certain videos when the object is moving continuously before a fixed background, but these methods can not be as generally used as learning system, which
can select the optimal template sequences from a larger set in runtime, based on the features of the tracked object and the features of the background.


 The goal of the selection is to minimize the difference between the ground-truth image (an image where all the pixels within the bounding box of the object are black and all the background pixels are white) and the weighted linear summation of descriptor images.

==> temp2.tex <==
\Note{Can this section be broken down into subsections?}

In this section, we provide a detailed description of the CeNN based target tracking algorithm.  The algorithm can be divided into two parts, training and tracking.

In the training part, a set of features are selected that best matches the target object and separates it from the features of the background and surrounding objects.  The feature pool is generated by running a user-specified number of kernels for features extraction (Difference of Gaussians - DoG and Gabor kernels) on an image and pooling the results. Each operation is defined by a pair of $3  \times 3$ A-templates. \Note{Can we/should we explain the CeNN mapping better?} A DoG kernel performs an isotropic or directional Gaussian diffusion generated from a unique covariance matrix and implements a band-pass filter. \note{The Gabor Kernels can identify different spatial frequencies depending on the orientation of the features. -- don't put it here}

The templates are paired with a time step count ranging from $10$ to $75$ (where 1 time step corresponds to $1ns$), and B-template and bias are set to zero. The runtime for CeNN is less than the settling time so an extra circuitry is needed to control the timing of diffusion. Only isotropic and directional diffusion are utilized to produce the feature set, which avoids the additional power overhead that would be incurred by non-linear anisotropic diffusion templates.

Following diffusion, CeNN is used to perform a SUBTRACTION operation as the final step for the DoG operation. Each DoG operation is followed by a pooling step, which also leverages fast-running CeNN templates. The most descriptive threshold is selected from a series of thresholds at different levels, and the binary result is diffused with an isotropic template. Together with the pooling operation, this step creates blobs from the extracted features. The result of this sequence of operations is a set of descriptor images with gray scale regions corresponding to different feature responses. This approach is similar to the operation used in deep learning, \Note{I think the connection to deep learning is a good idea!} but the binary output of a detected feature is diffused resulting a gray scale map encoding the location of the feature. In case of convolution network using max-pooling a binary map is provided.  \Note{This text does not really refer to the flow chart at all.  I think that would help!}

From this image set, a subset of descriptor images can be selected and weighed to create a globally sparse and high-response area corresponding to the estimated object position, given as a bounding box. A user-specified number of features is selected from the pool based on response strength within the bounding box.

The remaining features are then weighed by genetic algorithm, which employs the accuracy of the response with respect to the bounding box as its fitness function.  The goal of the selection is to minimize the difference between the ground-truth image (an image where all the pixels within the bounding box of the object are black and all the background pixels are white) and the weighted linear summation of descriptor images.  A fitness function ($F(I)$) is calculated as the are differences between the correctly and falsely classified pixels. expressed in the fitness function, where $I$ is the image generated by a vector of weights used to linearly sum the descriptors, $G$ is the ground truth, and $A$ is an area computation-
%\begin{equation}
%F(I) = A(G-I)
%\end{equation}

The amount of weight carried by the bounding box in the optimization problem (minimizing $F(I)$ across the linear sum of descriptors) is a function of its size relative to that of the image.  This reflects the difficulty of tracking smaller images in cluttered scenes.  A high response within the bounding box is prioritized (sometimes at the expense of a low background response), whereas a low background response is prioritized when the bounding box is larger.  After the genetic algorithm produces optimal linear weights, the linear sum of the descriptors is thresholded at a value that optimizes the same fitness function used in the genetic selection algorithm.

After training, the $3 \times 3$ Gaussian kernels, corresponding weights, and final threshold selected by the training process can be used as operators on subsequent images to identify the target. 

We leverage CeNN in the tracking part as a hardware accelerator. Part of the processing flow for tracking part is shown in Fig.\ref{tracking_algorithm}. The remaining part is Kalman filter-based processing which can be computed by the CPU.

\begin{figure}
    \centering
    \includegraphics[trim = 25mm 0mm 0mm 0mm, clip, width = 110mm]{Figs/tracking_algorithm.pdf}
    \caption{Processing flow for CeNN based tracking algorithm}
    \label{tracking_algorithm}
\end{figure}

Tracking is performed by taking the centroid of the local response area of the current frame and resizing the bounding box according to the dimensions of the response area relative to the response area of the first frame.  After the image is constructed, a THRESHOLD operation can be performed to convert the image into a binary one. A following AND operation with the ground truth image can extract the object of interest. Weak Kalman filtering is also utilized to estimate the motion of the object, while A Strong Kalman filter is used to resize the bounding box, which is more prone to fluctuation.

Although the calculation of DoG has an accuracy to be applied in practical problems \cite{collins2003mean,sinha2011feature} and these methods can extract meaningful features \cite{DoG}, it is observed in the field of computer vision and especially in deep learning that the application of Gabor kernels to extract meaningful features can further increase the detection accuracy for these applications \cite{GaborKernel}. By using Gabor kernels the algorithm will have an increased sensitivity to spatial frequencies and the orientation of edges. Some examples from the generated Gabor Filters can be seen on Fig \ref{GKernels}.

%figure of gabor kernels - not sure if it is needed though
\begin{figure}[t]
\includegraphics[width=8cm]{Figs/GaborFilters.png}
\centering
\caption{Some example filters can be seen on this image from the randomly generated filter bank, which were selected for feature extraction by the algorithm. As it can be seen, these filters are asymmetric and are able to compute gradients with different orientation. This orientation selectivity and asymmetry can result more specific features than the DoG kernels. }\label{GKernels}
\end{figure}

Once the extracted features are obtained, two SHADOW operations project the vertically and horizontally. The width and height of the bounding box of object can be easily calculated from this projections. We can use the assumption that the object moves only a limited number of pixels between two consecutive frames, thanks to this a DILATION operation is used to augment the possible location of the tracked object. The amount of the dilation is exactly the number of pixels which the object could move. This map can help in the localization of the object on the next frame, because we can assure that the tracked object will appear in the dilated region. Once the bounding box was obtained Kalman filter algorithm is applied by the CPU to predict the motion of the object and to smooth the noise obtained by the position estimation. Once the position estimation is known the second part of the algorithm is executed on the next frames iteratively.

\Note{Are these last two paragraphs referring to techniques that you used for just 1 sequence to show improvement in accuracy?  If so, I would reduce and move this text to a later point in the paper.  I still am not sure I see the value in Fig. \ref{GKernels}.}

%Furthermore, the training process can easily be extended to perform high-level feature extraction and general classification tasks in the future.


==> temp3.tex <==
\Note{Can this section be broken down into subsections?}

In this section, we provide a detailed description of the CeNN based target tracking algorithm.  The algorithm can be divided into two parts, training and tracking.

\subsection{Training}
The training part is an offline process, we do the processing in CPU. A set of features are selected that best matches the target object and separates it from the features of the background and surrounding objects. The feature pool is generated by running a user-specified number of kernels for features extraction (Difference of Gaussians - DoG) on an image and pooling the results. A DoG kernel performs two isotropic or directional Gaussian diffusions along with a substraction operation. Each DoG kernel is paired with a time step count ranging from $10$ to $75$ (where 1 time step corresponds to $1ns$).  The DoG can be realized via CeNN operation. Each diffusion operation is defined by a pair of $3  \times 3$ A-templates in CeNN configuration, while B-template and bias are zero. 
Following diffusion, CeNN is also used to perform a SUBTRACTION operation. 

Each DoG operation is followed by a pooling step, which also leverages fast-running CeNN templates. The most descriptive threshold is selected from a series of thresholds at different levels, and the binary result is diffused with an isotropic template. Together with the pooling operation, this step creates blobs from the extracted features. The result of this sequence of operations corresponds to different feature responses. This approach is similar to the operation used in deep learning, \Note{I think the connection to deep learning is a good idea!}  \Note{This text does not really refer to the flow chart at all.  I think that would help! (This is for training... The flow chart is for tracking)}

From this image set, a subset of descriptor images can be selected and weighed to create a globally sparse and high-response area corresponding to the estimated object position, given as a bounding box. A user-specified number of features is selected from the pool based on response strength within the bounding box.

The remaining features are then weighed by genetic algorithm.  The goal of the selection is to minimize the difference between the ground-truth image (an image where all the pixels within the bounding box of the object are black and all the background pixels are white) and the weighted linear summation of descriptor images. After the genetic algorithm produces optimal linear weights, the linear sum of the descriptors is thresholded at a value that optimizes the same fitness function used in the genetic selection algorithm.

After training, the $3 \times 3$ Gaussian kernels, corresponding weights, and final threshold selected by the training process can be used as operators on subsequent images to identify the target. 

\subsection{Tracking}
We leverage CeNN in the tracking part as a hardware accelerator to execute these CeNN-friendly operations. Part of the processing flow for tracking part is shown in Fig.\ref{tracking_algorithm}. The remaining part is Kalman filter-based processing which can be computed by the CPU.

\begin{figure}
    \centering
    \includegraphics[trim = 25mm 0mm 0mm 0mm, clip, width = 110mm]{Figs/tracking_algorithm.pdf}
    \caption{Processing flow for CeNN based tracking algorithm}
    \label{tracking_algorithm}
\end{figure}

The pre-defined DoG kernels are used in the tracking to profile the interest object. Since DoG kernels are weighted by generic algorithm, the weighted sum of image after DoG would be the featured image.
The runtime for each DoG operation is less than the settling time of CeNN, so an extra circuitry is needed to control the timing of operation.
Then, tracking is performed by taking the centroid of the local response area of the current frame and resizing the bounding box according to the dimensions of the response area relative to the response area of the first frame.  After the image is constructed, several CeNN operations follow. A THRESHOLD operation can be performed to convert the image into a binary one. A following AND operation with the ground truth image can extract the object of interest. Once the extracted features are obtained, two SHADOW operations project the vertically and horizontally. The width and height of the bounding box of object can be easily calculated from this projections. A DILATION operation is used to augment the possible location of the tracked object, to ensure object moves only a limited number of pixels between two consecutive frames. In the second part, the CPU applies two Kalman filters. Weak Kalman filtering is also utilized to estimate the motion of the object, while A Strong Kalman filter is used to resize the bounding box, which is more prone to fluctuation.
Once the position estimation is known the second part of the algorithm is executed on the next frames iteratively.

\Note{Are these last two paragraphs referring to techniques that you used for just 1 sequence to show improvement in accuracy?  If so, I would reduce and move this text to a later point in the paper.  I still am not sure I see the value in Fig. \ref{GKernels}.}

%Furthermore, the training process can easily be extended to perform high-level feature extraction and general classification tasks in the future.

